Network and Physical Layer Attacks and countermeasures to AI-Enabled 6G O-RAN

Artificial intelligence (AI) will play an increasing role in cellular network deployment, configuration and management. This paper examines the security implications of AI-driven 6G radio access networks (RANs). While the expected timeline for 6G standardization is still several years out, pre-standardization efforts related to 6G security are already ongoing and will benefit from fundamental and experimental research. The Open RAN (O-RAN) describes an industry-driven open architecture and interfaces for building next generation RANs with AI control. Considering this architecture, we identify the critical threats to data driven network and physical layer elements, the corresponding countermeasures, and the research directions.

==> Ref_discuss.tex <==
R(1): Introduction Ref for security
R(2,3): GIO comments as suggestions in the introduction.



-R(4): Jamming prevention (general approach to reduce the effect of jamming by adding redundancy) (old paper) --> not important



R(5): Spoofing prevention ( support ref to one of our new approaches, not included UAV but the technique used there can be applied on our UAV proposal(new paper)) --> semi important

R(6): Spoofing prevention ( support ref to one of our new GPS relaying approaches, include UAV) (new paper) -->  important



R(7): Eavesdropping detection (support ref to sense leakage of the Rf to help detecting the eavesdropper, not included UAV but the technique can be used on the UAV approach (old proposal)) --> semi important (Gio don't believe)


R(8): Eavesdropping detection (support ref to features that can be used to help detecting the eavesdropper, not included UAV but the technique can be used on the UAV (new  paper)) --> semi important 


R(9): Jamming detection  (support ref of spectrum sensing technique that can be used to help detecting the jammer, not included UAV but the technique can be used on the UAV (new  paper)) --> semi important

REMOVE SOME OF THEM, VERY OLD: R(10,11,12,13):  Jamming detection (support refs as some range-based and range free that can be used to help detecting the jammer, not included UAV but the technique can be used on the UAV (new  paper)) --> semi important (don't know if we need all of them or not)

R(14): Jamming detection  (support ref as an example of using distributed or centralized jamming detection techniques, not included UAV but the technique can be used on the UAV (old  paper)) --> semi important ( this to elaborate that can be used over swarm of UAVS or single UAVs)

-R(15): jamming detection ( localization of jammers in UAVs network) (old paper) --> not important



-R(16): Spoofing detection (general approach to user virtual channel modeling over 5G for localize the spoofing) (old paper) --> not important

R(17): Spoofing detection (UAV approach to use other UAVS measurements information to localize the spoofer) (old paper) --> semi important

R(18): Spoofing detection  (support ref of spectrum sensing technique that can be used to help detecting the spoofer, not included UAV but the technique can be used on the UAV (new  paper)) --> semi important



R(19): Eavesdropping recovery (support ref that discuss the use of aerial rely, resource allocation, and path trajectory to overcome the eavesdropping , include UAV (old  paper)) -->  important



R(20):Jamming recovery (support ref that discuss the use of aerial rely to overcome the jamming in VANET using UAV , include UAV (old  paper)) -->  important or semi important based on the discussion of Gio comment about relay similarity approaches ( a replacement can be the hot zone idea)


R(21):Jamming recovery (support ref that discuss the use of 3D beamforming and UAV positioning to mitigate the jammer using UAV , include UAV (old  paper)) -->  important ( zhang paper that was one of the reviewer's comment) 


R(22):spoofing recovery (support ref that discuss the use of UAV positioning to mitigate the gps spoofing, include UAV (old  paper)) -->  semi important ( maybe relative to the UAV's GPS relaying idea)


R(23): A2A channel model ref 


R(3): Gio's Ref --> 3GPP LTE-UAV report


R(24): AERPAW 



==> include/KPI_table.tex <==
\begin{table}[ht]
\centering
\caption{\hl{This Table may be removed} 6G vs. 5G KPI}
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{5.5cm}|p{0.8cm}|p{0.8cm}|}
\hline
\centering \textbf{KPI} & \centering \textbf{5G} &  \textbf{\hspace{1 pt} 6G}
\\ \hline
\vspace{0.001 in}
Peak Data Rate (Gbps) &

\vspace{-0.05 in}
10 
\vspace{-0.1 in}

&
\vspace{-0.05 in}
1000 
\vspace{-0.1 in}


\\ \hline

\vspace{0.001 in}
Experienced Data Rate (Gbps) &

\vspace{-0.05 in}
0.1 
\vspace{-0.1 in}

&
\vspace{-0.05 in}
1 
\vspace{-0.1 in}


\\ \hline
\vspace{0.001 in}
E2E Latency  (ms)&

\vspace{-0.05 in}
1 
\vspace{-0.1 in}

&
\vspace{-0.05 in}
0.1 
\vspace{-0.1 in}

\\ \hline
\vspace{0.001 in}
Maximum Channel Bandwidth (GHz) &

\vspace{-0.05 in}
1
\vspace{-0.1 in}

&
\vspace{-0.05 in}
100
\vspace{-0.1 in}

\\ \hline
\vspace{0.001 in}
Peak Spectral Efficiency (b/s/Hz) &

\vspace{-0.05 in}
30
\vspace{-0.1 in}

&
\vspace{-0.05 in}
60
\vspace{-0.1 in}
\\ \hline
\vspace{0.001 in}
Connection density (devices/km^{2}) &

\vspace{-0.05 in}
10^{6}
\vspace{-0.1 in}

&
\vspace{-0.05 in}
10^{7}
\vspace{-0.1 in}
\\ \hline
\vspace{0.001 in}
Area Traffic Capacity(Mbps/m^{2}) &

\vspace{-0.05 in}
10
\vspace{-0.1 in}

&
\vspace{-0.05 in}
1000
\vspace{-0.1 in}
\\ \hline
\vspace{0.001 in}
Reliability (Packet Error Rate) &

\vspace{-0.05 in}
10^{-5}
\vspace{-0.1 in}

&
\vspace{-0.05 in}
10^{-9}
\vspace{-0.1 in}
\\ \hline
\vspace{0.001 in}
Mobility (km/h) &

\vspace{-0.05 in}
500
\vspace{-0.1 in}

&
\vspace{-0.05 in}
1000
\vspace{-0.1 in}
\\ \hline
\end{tabular}%
}

\label{tab:KPI}
\end{table}

==> include/ORANusecasesTable.tex <==
\begin{table*}[ht]
\centering
\caption{\h{Representative O-RAN use cases where AI will be employed.}}
\footnotesize
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{1.5cm}|p{0.9cm}|p{3cm}|p{1.4cm}|p{1.4cm}|p{4.4cm}|p{2.4cm}|}
\hline
 \textbf{Use Case} &\textbf{Network Layer} &  \textbf{AI models functionality description}  &   \textbf{AI training host}  & \textbf{AI infe-rence host }  &   \textbf{Training data}  &  \textbf{Action} 

\\ \hline
%\vspace{0.001 in} 
Massive MIMO beamforming optimization 
& PHY  
& Predict the optimal configuration of Massive MIMO parameters for each cell according to a global optimization objective designed by the operator. 
&  Non-RT RIC &  Non-RT RIC 
& KPI related to traffic load, coverage and QoS performance, per beam/area and massive MIMO configuration.
& Configure the optimized beam parameters via the O1 interface.
\\ \hline

%\vspace{0.001 in}
Quality of experience (QoE) optimization 
& MAC  
& %Making predictions on
Predict the application/traffic types, QoE and available bandwidth. 
& Non-RT RIC 
& Near-RT RIC 
& Network level measurement report including UE data, L2 measurement, RAN protocol stack status, cell level information, QoE measurement metrics and user traffic. 
& E2 control or policy commands towards RAN for QoE optimization.
\\ \hline

%\vspace{0.001 in} 
Dynamic spectrum sharing 
& MAC  
& Predict the short-
term traffic demand %for 4G and 5G network 
based on near real time metrics from the RAN. 
& non-RT DSS-App 
& DSS xApps at near-RT RIC 
& Geography location, DSS modality, cell configuration information, PRB used/reserved/requested/blocked, bitmap information, number of active UEs, traffic demand, QoS classes, UE capability and UE location information 
& E2 control/policy of resources configuration and scheduling coordination.
\\ \hline

%\vspace{0.001 in} 
Network slice subnet instance (NSSI) resource allocation optimization 
& MAC  
& Predict of the traffic demand patterns of NSSI at different times and locations 
& Non-RT RIC & NA 
& Measurement counters per slicing subnet instance. These  include DL and UL PHY resource blocks (PRBs) used for data traffic, average DL and UL throughput, % in gNB average UL UE throughput in gNB, 
and the number of packet data unit (PDU) sessions requested, % to setup, Number of PDU sessions 
successfully set up and %number of PDU sessions 
failed to set up 
& Reconfigure the NSSI attributes via the O1 interface and update the Cloud resources via the O2 interface.
\\ \hline
\end{tabular}%
}

\label{tab:ORANuse}
\end{table*}
\lable

==> include/ServicesTable.tex <==
\begin{table*}[ht]
\centering
\caption{\hl{Include into Fig. 1} 6G Services}
%\resizebox{0.85\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|}
{\begin{tabular}{|p{0.95cm}|p{3.8cm}|p{3.8cm}|p{2.8cm}|}
\hline
 \textbf{Service} &  \textbf{Technology Enablers} &  \textbf{Main KPIs}  &  \textbf{Sample use cases}
\\ \hline
\vspace{0.001 in}
URLLC &

\vspace{-0.05 in}
Network slicing, NOMA, ME computing and caching, Intelligence, short TTI, and Grant free transmission and scheduling  


&
--


&

VR, AR, XR, Holographic 

\\ \hline

\vspace{0.001 in}
uMBB &


Ultra massive MIMO, RIS, Cell free, Heterogeneous network, mmWave, THz, Optical, NOMA, and Intelligence

&
--


&

Tactical IoT

\\ \hline
\vspace{0.001 in}
mMTC &


Grant free transmission and scheduling, NOMA, Adaptive scheduling, SDN, NFV, ME computing and caching, SWIPT, Network Slicing, and Intelligence

&
Connection density: $10^5$ to $10^7$ (devices/km2) 

Packet loss probability: $10^−5 $ to $10^−9$

Availability: 99.9999\% 

Latency: 1 ms
&

Autonomous Intelligent Driving, Industrial IoT, and Remote Surgery


\\ \hline
\end{tabular}%
}

\label{tab:Services}
\end{table*}

==> include/case.tex <==

\textcolor{red}{Describe the killer applications and their requirements (KPIs)
Also their security requirements since the focus is on security.}



==> include/contribution2.tex <==




























==> include/directions_v2.tex <==

\begin{itemize}
    \item Security in the era of Quantum Computing: ....
    \item ....
    \item ...
    
\end{itemize}

==> include/oran_usecases.tex <==
 \subsection{O-RAN ML based use cases and attacks}
 Introducing the O-RAN in 6G makes the radio access network more Intelligent based and open comparing to the current deployment radio access network. The intelligent part of the O-RAN is based on utilize some ML/AL model and the open interfaces  for RAN elements and resources optimizations to meet the requirements of the increasingly complex, denser and more heterogeneous future wireless network. The O-RAN architecture supports three different control loops loop 1(O-DU Scheduler control loop), loop 2 (Near-RT RIC control loop) and loop 3 (Non-RT RIC control loop). The defining of the control loop is based in the entity being controlled and the timing requirement for the controlling. The three control loop run in parallel and could depends on each other based on the used case.  The ML model could be used to assist one or more of these control loops based in the parameters needed to be optimized and controlled. Three different deployment scenarios that are considered for ML architecture/framework in O-RAN architecture based on the training and inference hosts, scenario 1 where the Non-RT RIC acts as both the ML training and inference host, scenario 2 Non-RT RIC acts as the ML training host and the Near-RT RIC as the ML inference host and scenario 3 Non-RT RIC acts as the ML training host and the O-CU/O-DU as the ML inference host. Choose of deployment scenario depends on different criteria such as the Computation complexity and resources availability of the model, training data type and availability across a given interface, the latency consideration and the cost of the data movement over the interfaces. 
O-RAN Alliance described in Work Grope 1 (WG1) specifications different use cases that leverage the O-RAN architecture and demonstrate its unique benefits to optimize a RAN function and update policies based on performance measurement. some of these used cases deploy one of the aforementioned ML deployment scenario in the O-RAN architecture. Table~\ref{tab:ORANus} provides details about each one of these use cases.
\begin{itemize}
    \item \textbf{QoE Optimization}: this use case automates the configuration and controlling of RAN parameters to improve the QoE of the user by utilizing the intelligent and open interface of the O-RAN architecture. The limited radio resources are utilized in a way that the  UE's use specific applications that requires critical KPI e.g. Cloud VR assign sufficing radio resources to meet these KPI and improve there QoE. The ML solution for this case consists of training model at the Non-RT RIC to obtain QoE related models such as Application Classification Model, QoE Prediction Model, QoE policy Model and Available BW Prediction Model. The offlkine model will use the training data data in table~\ref{tab:ORANus} which provided by the E2 node over the O1 interface. After the training phase, the QoE related ML model will be deployed in Near- RT RIC to assist in the QoE Optimization function. The Near- RT RIC
\end{itemize}


